Sampling from Pre-Images to Learn Heuristic Functions for Classical Planning

We introduce a new algorithm, Regression based Supervised Learning (RSL), for learning per instance Neural Network (NN) defined heuristic functions for classical planning problems. RSL uses regression to select relevant sets of states at a range of different distances from the goal. RSL then formulates a Supervised Learning problem to obtain the parameters that define the NN heuristic, using the selected states labeled with exact or estimated distances to goal states. Our experimental study shows that RSL outperforms, in terms of coverage, previous classical planning NN heuristics functions while requiring two orders of magnitude less training time.

==> macros.tex <==
% % Environments and Theorems
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%% General Math


\newcommand{\conv}[1]{$\mathit{conv(#1)}$}

\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}} 
%\newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}

\newcommand{\BE}{{\mathcal{B}, \mathcal{E}}} 

\newcommand{\TAU}{\mathcal{T}} 

\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\sub}[1]{[#1]}
\newcommand{\tup}[1]{\langle #1\rangle}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

\newcommand{\pv}[1]{#1^{b}}
\newcommand{\sv}[1]{#1^{d}}

\newcommand{\hpp}{ \langle \pv{X},\sv{X},D,s_0,A,G,C \rangle }


% % % Names of things, acronyms, software, etc.
\newcommand{\propername}[1]{\text{\textsf{\small #1}}\xspace}

\newcommand{\PDDL}{\textsc{pddl}}
\newcommand{\PDDLplus}{\textsc{pddl}$+$}
\newcommand{\PDDLPlus}{\textsc{pddl}$+$}
\newcommand{\FPDDL}{$\smallint$-\textsc{pddl}$+$}
\newcommand{\ADL}{\textsc{adl}}
\newcommand{\FS}{\propername{FS}}
\newcommand{\FSTRIPS}{FSTRIPS}
\newcommand{\SMT}{\textsc{Smt}}
\newcommand{\SAT}{\textsc{Sat}}
\newcommand{\CP}{\textsc{Cp}}
\newcommand{\FMSMT}{\propername{FM-SMT}}
\newcommand{\HSHP}{\propername{HSHP}}
\newcommand{\CNF}{\propername{CNF}}
\newcommand{\Zthree}{\propername{Z3}}
\newcommand{\MathSat}{\propername{MathSAT}}
\newcommand{\LpSat}{\propername{LPSAT}}
\newcommand{\TmLpSat}{\propername{TM-LPSAT}}
\newcommand{\Colin}{\propername{COLIN}}
\newcommand{\PSR}{\textsc{Psr}}
\newcommand{\HBW}{\textsc{Hbw}}
\newcommand{\FF}{\propername{FF}}
\newcommand{\MetricFF}{\propername{MetricFF}}
\newcommand{\FSZero}{\propername{FS0}}
\newcommand{\FSPlus}{\propername{FS+}}
\newcommand{\LTI}{\textsc{Lti}}
\newcommand{\HA}{\textsc{Ha}}
\newcommand{\UPMurphi}{\propername{UPMurphi}}
\newcommand{\Dino}{\propername{DiNo}}
\newcommand{\dreal}{\propername{dReal}}
\newcommand{\Convoys}{\textsc{Convoys}}
\newcommand{\ENHSP}{\propername{ENHSP}}

\newcommand{\Kongming}{\propername{Kongming}}
\newcommand{\GraphPlan}{\propername{GraphPlan}}
\newcommand{\SpaceEx}{\propername{SpaceEx}}
\newcommand{\ode}{\textsc{ode}}
\newcommand{\blind}{\textsc{Brfs}}
\newcommand{\uct}{\textsc{Uct}}
\newcommand{\iwk}{\textsc{IW}($k$)}
\newcommand{\PNE}{\propername{PNE}}
\newcommand{\Fstrips}{\textsc{FSTRIPS}}
\newcommand{\FOL}{\textsc{FOL}}
\newcommand{\MPC}{\textsc{MPC}}
\newcommand{\TFD}{\propername{TFD}}
\newcommand{\AIBR}{\textsc{Aibr}}
\newcommand{\RRT}{\textsc{RRT}}
\newcommand{\SMTPlan}{\textsc{SMTPlan+}}


\newcommand{\Car}{\textsc{Car, Linear}}
\newcommand{\NLCar}{\textsc{Car, Nonlinear}}
\newcommand{\CarSC}{\textsc{Car, Linear, State Constraints}}
\newcommand{\NLCarSC}{\textsc{Car, Nonlinear, State Constraints}}
\newcommand{\Generator}{\textsc{Generator, Linear}}
\newcommand{\NLGenerator}{\textsc{Generator, Nonlinear}}
\newcommand{\Agile}{\textsc{Agile Robot}}
\newcommand{\Orbital}{\textsc{Orbital Rendezvous}}
\newcommand{\Descent}{\textsc{1D Powered Descent}}
\newcommand{\Intercept}{\textsc{Intercept}}
\newcommand{\Zermelo}{\textsc{Zermelo}}

% % formulas

\newcommand{\f}[1]{\sum_{r=0}^{m}\alpha_{{#1},t_0}^r e_{#1,t_0} + 
	\alpha_{#1,t_0}^m x_{#1}}
\newcommand{\ft}[2]{\alpha^m #1 + \sum_{r=0}^{m}\alpha^r (\sum_{i} w_i x_i + k)}
\newcommand{\ftm}[3]{\sum_{r=0}^{#3}\alpha_{{#1},#2}^r e_{#1,#2} + 
	\alpha_{#1,#2}^{#3} x_{#1}}

\newcommand{\eminus}{\sum_{j\neq i}w_j x^{i}_j + k}


\newcommand{\ftms}[3]{f_{#1}^{#2}(#3)}

\newcommand{\alphaf}[2]{\alpha_{{#1},#2}}

\newcommand{\pre}[1]{\ensuremath{\mathrm{pre}_{#1}}}
\newcommand{\eff}[1]{\ensuremath{\mathrm{eff}_{#1}}}
\newcommand{\action}[1]{\Tup{ \pre{#1}, \eff{#1} }}
\newcommand{\prop}[1]{{\cal P}_{A}}
\newcommand{\matr}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\invmatr}[1]{\mathbf{#1}^{-1}}
\newcommand{\transmatr}[1]{\mathbf{\Phi}(#1)}
\newcommand{\Matlab}{\propername{Matlab}}
\newcommand{\Octave}{\propername{Octave}}
\newcommand{\Sympy}{\propername{SymPy}}
\newcommand{\Mathematica}{\propername{Mathematica}}
\newcommand{\relproc}[2]{{\cal P}_{#1|x_{#2}}}
\newcommand{\MBP}{\propername{MBP}}
\newcommand{\OpTop}{\propername{OpTop}}
\newcommand{\Mode}[1]{{\cal M}(\matr{#1})}	
\newcommand{\ProcExpr}[2]{\xi_{x_{#1}|#2}(\matr{x})}
\newcommand{\Affected}[1]{\mathrm{aff}({#1})}
\newcommand{\Proc}[1]{\ensuremath{\mathrm{proc}(#1)}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}

\newcommand{\Pong}{\textsc{Pong}}
\newcommand{\UCT}{\textsc{UCT}}
\newcommand{\BRFS}{\textsc{BrFS}}
\newcommand{\IW}[1]{\textsc{IW}$(#1)$}

\newcommand{\thereals}{\ensuremath{\mathbb{R}}}

\newcommand{\hzero}[1]{$s_{0}^{h_{#1}}$}
\newcommand{\hfinal}[1]{$s_{f}^{h_{#1}}$}
% Variants of the two macros above to be embedded in
% math mode
\newcommand{\mhzero}[1]{s_{0}^{h_{#1}}}
\newcommand{\mhfinal}[1]{s_{f}^{h_{#1}}}

\newcommand{\tzero}[1]{$T_{0}^{h_{#1}}$}
\newcommand{\tfinal}[1]{$T_{f}^{h_{#1}}$}
% Variants of the two macros above to be embedded in
% math mode
\newcommand{\mtzero}[1]{T_{0}^{h_{#1}}}
\newcommand{\mtfinal}[1]{T_{f}^{h_{#1}}}
\newcommand{\hinvar}[1]{${\cal I}^{h_{#1}}$}
\newcommand{\LP}{\propername{LP}}

\newcommand{\Rplus}{R^{+}}
\newcommand{\Rminus}{R^{-}}
\newcommand{\Vplus}{V^{+}}
\newcommand{\Vminus}{V^{-}}

\newcommand{\varmode}{\ensuremath{\textbf{ctl}}}
\newcommand{\litleft}{\ensuremath{\text{left}}}
\newcommand{\litstraight}{\ensuremath{\text{straight}}}
\newcommand{\litright}{\ensuremath{\text{right}}}

\newcommand{\rkfs}{\propername{FS+}$_{RK22}$}
\newcommand{\rkfsnv}{\propername{FS+}$_{RK22,NV}$}

\newcommand{\AStar}{\ensuremath{\text{A}^*}}

\sisetup{
	round-mode          = places, % Rounds numbers
	round-precision     = 2, % to 2 places
}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\VAL}{\propername{Val}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\matt}[1]{\ensuremath{\mathbf{#1}^{T}}}
\newcommand{\Useq}{\ensuremath{\mathbf{U}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}

==> packages.tex <==
\usepackage{times}  %Required
\usepackage{helvet}  %Required
\usepackage{courier}  %Required
\usepackage{url}  %Required
\usepackage{graphicx}  %Required

\usepackage{enumitem} % Customized lists
\setlist[itemize]{noitemsep} % Make itemize lists more compact
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}

\usepackage{latexsym}
\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{url}
\usepackage{xspace}
\usepackage{soul}
\usepackage{todonotes}
%% for nice underlying \ul{xxx}
\setuldepth{x} 
%\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{todonotes}
\usepackage{filecontents}
%\usepackage{stmaryrd}

% \renewcommand{\baselinestretch}{.99}
\usepackage{tikz}
\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{longtable}
\usepackage{array}
\usepackage{colortbl}
\usepackage{booktabs} % For \toprule, \midrule and \bottomrule
\usepackage{siunitx} % Formats the units and values
\usepackage{pgfplotstable} % Generates table from .csv
%\usetikzlibrary{arrows,decorations,backgrounds,automata,shapes,patterns,decorations,backgrounds,plotmarks,calc,fit}
\usetikzlibrary{arrows,decorations,backgrounds,automata,shapes,patterns,decorations,backgrounds,plotmarks,calc,fit,positioning}

% NIPS Specific, note this stuff isn't liked by AAAI or IJCAI!
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
